Boosting human decision-making with AI-generated decision aids

Human decision-making is plagued by many systematic errors. Many of these errors can be avoided by providing decision aids that guide decision-makers to attend to the important information and integrate it according to a rational decision strategy. Designing such decision aids used to be a tedious manual process. Advances in cognitive science might make it possible to automate this process in the future. We recently introduced machine learning methods for discovering optimal strategies for human decision-making automatically and an automatic method for explaining those strategies to people. Decision aids constructed by this method were able to improve human decision-making. However, following the descriptions generated by this method is very tedious. We hypothesized that this problem can be overcome by conveying the automatically discovered decision strategy as a series of natural language instructions for how to reach a decision. Experiment 1 showed that people do indeed understand such procedural instructions more easily than the decision aids generated by our previous method. Encouraged by this finding, we developed an algorithm for translating the output of our previous method into procedural instructions. We applied the improved method to automatically generate decision aids for a naturalistic planning task (i.e., planning a road trip) and a naturalistic decision task (i.e., choosing a mortgage). Experiment 2 showed that these automatically generated decision-aids significantly improved people's performance in planning a road trip and choosing a mortgage. These findings suggest that AI-powered boosting might have potential for improving human decision-making in the real world.

==> figures.tex <==
\newcommand{\figSD}{
\begin{figure}[b]
    \centering
    \includegraphics[width=0.9\linewidth]{general_SD.png}
    \caption{AI-powered boosting relies on discovering optimal decision strategies by modeling decision problems as a metalevel Markov Decision Process and solving them with metalevel reinforcement learning \citep{Griffiths2019}}
    \label{fig:SD}
\end{figure}
}

\newcommand{\figEnvs}{
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.8\linewidth]{envs2.png}
    \caption{Naturalistic decision-tasks used in Experiment~2. \textbf{a}: In the Road Trip task, the objective is to efficiently find an inexpensive route to a city with an airport. Participants can use a search engine to look up how costly it is to spend the night in different cities. \textbf{b}: In the Mortgage task the goal is to choose the most affordable mortgage by considering interest rates for different time horizons. Participants can learn about the interest rates by clicking on appropriate boxes}
    \label{fig:envs}
\end{figure}
}

\newcommand{\figMouselab}{
\begin{figure}
\centering
\includegraphics[width=0.55\linewidth]{flight_planning.png}
\caption{Mouselab-MDP with increasing variance. Nodes in the Mouselab-MDP represent short-, mid-, and long-term consequences of potential actions where the black node is the starting position, and connections in the Mouselab-MDP symbolize ``possible later consequence'' relation. Information on the consequences is represented numerically as rewards, and can be acquired by clicking on the nodes. Rewards are drawn from a normal distribution whose variance increases with the distance of the node from the starting node.  Thus, rewards that are farthest from the starting position (long-term consequences) show the highest variance. As gathering information is costly, the agent's goal in the Mouselab-MDP is to make as few clicks as possible to uncover the best possible course of actions with the highest total reward}
\label{fig:mouselab}
\end{figure}
}

\newcommand{\figFlowchart}{
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.7\linewidth]{DT1.png}
    \caption{Sample flowchart obtained via the AI-powered boosting intervention from \citep{skirzynski2020automatic}. The flowchart expresses a far-sighted planning strategy in the Mouselab-MDP task with increasing variance}
    \label{fig:flowchart}
\end{figure}
}


\newcommand{\figExpOneTask}{
\begin{figure}[h!]
\begin{center}
\includegraphics[width=0.99\linewidth]{expProc_task.png}
\end{center}
\caption{Experiment 1: The experimental screen as shown to participants in the flowchart condition. On the right, the Mouselab-MDP task with color coded nodes. Each color represents a node property, which can change depending on the uncovered values. On the right, the color coded flowchart depicting a specific clicking procedure. In the alternative condition the flowchart is replaced with procedural instructions}
\label{fig:exp1_task}
\end{figure}
}

\newcommand{\figExpOneResults}{
\begin{figure}[h!]
\begin{center}
\includegraphics[width=1\linewidth]{Exp1_results_extended.pdf}
\end{center}
\caption{Experiment 1: a) Procedural instructions are more interpretable than static descriptions (\textit{p}=.018). The plot shows the mean click agreement of participants of the experimental conditions (blue and red) and a control condition (grey).  b) Participants assisted by procedural instructions had higher expected scores than participants assisted by static descriptions (\textit{p}=.09). The expected score that participants would have received if they had performed their clicks in the Mouselab-MDP task
}
\label{fig:exp1_results}
\end{figure}
}


\newcommand{\figExpOneLearningCurves}{
\begin{figure}[h!]
\begin{center}
\includegraphics[width=1\linewidth]{Exp1_learningcurves.pdf}
\end{center}
\caption{Experiment 1: a) Procedural instructions are more interpretable than flowcharts. The plot shows the mean click agreement of participants per condition as a function of trial. Click agreement with the instructed clicking strategy was measured as the proportion of consistent clicks out of all performed clicks. b) The mean expected score that per condition as a function of trial. The shaded areas mark the 95\% confidence intervals
}
\label{fig:exp1_learningcurves}
\end{figure}
}

\newcommand{\figExpTwoResults}{
\begin{figure}[h!]
\begin{center}
\includegraphics[width=0.90\linewidth]{Exp2_combined.pdf}
\end{center}
 \vspace{-18pt}
\caption{Results of Experiment 2. The decision aids generated by our AI method boosted participants far-sightedness and performance in the Road Trip and Mortgage task. The experimental group was aided by the procedural instructions generated by our computational method. All differences are statistically significant (all $p \leq .01$).\\
Panels a-b: The experimental group planned more far-sighted than the control group. Panels c-d: The experimental group achieved higher click agreements than the control group. Panels e-f: Performance in both tasks was measured according to each task's objective. Higher scores mean better performance}
\label{fig:exp2_results}
\end{figure}
}

\newcommand{\figExpTwoTasks}{
\begin{figure}%[b]
\begin{center}
\includegraphics[width=0.9\linewidth]{Exp2_tasks2.png}
\end{center}
\caption{Experiment 2: The Road Trip task (a) and the Mortgage task (b) with corresponding AI-generated decision aids as presented to the experimental condition. Only participants in the experimental condition were assisted with decision aids}
\label{fig:exp2_tasks}
\end{figure}
}

\newcommand{\figExpTwoLearningCurves}{
\begin{figure}[h!]
\begin{center}
\includegraphics[width=1\linewidth]{Exp2_learning_curves.pdf}
\end{center}
\caption{Experiment 2: The experimental group (red) was supported by our decision aid whereas the control group (blue) was not. a) The plot shows the average far-sightedness quotient as a function of trial per condition for the Mortgage task. b) The plot shows the average far-sightedness quotient as a function of trial per condition for the Road Trip task. c) The plot shows the proportion of optimal choices as a function of trial per condition for the Mortgage task. b) The plot shows the average score as a function of trial per condition for the Mortgage task. The shaded areas mark the 95\% confidence intervals
}
\label{fig:exp2_learningcurves}
\end{figure}
}


\newcommand{\figISD}{
\begin{figure}%[h!]
\begin{center}
\includegraphics[width=0.99\linewidth]{AI_boosting.png}
\end{center}
\caption{AI-powered boosting with decision aids conveys automatically found planning strategies through automatically generated procedural instructions. Automation in the former area is achieved by modeling the problem as a metalevel MDP and solving it with metalevel reinforcement learning. Automation in the latter area rests on i) utilizing an imitation learning algorithm AI-Interpret that constructs a DNF formula of predefined predicates to describe the strategy, ii) applying the DNF2LTL method that transforms the DNF into a formula in LTL, iii) translating the output into natural langauge using a pre-defined predicate-to-expression dictionary}
\label{fig:isd}
\end{figure}
}

